JUNO Physics and Detector

The Jiangmen Underground Neutrino Observatory (JUNO) is a 20 kton LS detector at 700-m underground. An excellent energy resolution and a large fiducial volume offer exciting opportunities for addressing many important topics in neutrino and astro-particle physics. With 6 years of data, the neutrino mass ordering can be determined at 3-4 sigma and three oscillation parameters can be measured to a precision of 0.6% or better by detecting reactor antineutrinos. With 10 years of data, DSNB could be observed at 3-sigma; a lower limit of the proton lifetime of 8.34e33 years (90% C.L.) can be set by searching for p->nu_bar K^+; detection of solar neutrinos would shed new light on the solar metallicity problem and examine the vacuum-matter transition region. A core-collapse supernova at 10 kpc would lead to ~5000 IBD and ~2000 (300) all-flavor neutrino-proton (electron) scattering events. Geo-neutrinos can be detected with a rate of ~400 events/year. We also summarize the final design of the JUNO detector and the key R&D achievements. All 20-inch PMTs have been tested. The average photon detection efficiency is 28.9% for the 15,000 MCP PMTs and 28.1% for the 5,000 dynode PMTs, higher than the JUNO requirement of 27%. Together with the >20 m attenuation length of LS, we expect a yield of 1345 p.e. per MeV and an effective energy resolution of 3.02%/\sqrt{E (MeV)}$ in simulations. The underwater electronics is designed to have a loss rate <0.5% in 6 years. With degassing membranes and a micro-bubble system, the radon concentration in the 35-kton water pool could be lowered to <10 mBq/m^3. Acrylic panels of radiopurity <0.5 ppt U/Th are produced. The 20-kton LS will be purified onsite. Singles in the fiducial volume can be controlled to ~10 Hz. The JUNO experiment also features a double calorimeter system with 25,600 3-inch PMTs, a LS testing facility OSIRIS, and a near detector TAO.

==> JUNOauthors.tex <==
Angel Abusleme$^{5}$,
Thomas Adam$^{45}$,
Shakeel Ahmad$^{66}$,
Rizwan Ahmed$^{66}$,
Sebastiano Aiello$^{55}$,
Muhammad Akram$^{66}$,
Fengpeng An$^{29}$,
Guangpeng An$^{10}$,
Qi An$^{22}$,
Giuseppe Andronico$^{55}$,
Nikolay Anfimov$^{67}$,
Vito Antonelli$^{57}$,
Tatiana Antoshkina$^{67}$,
Burin Asavapibhop$^{71}$,
Jo\~{a}o Pedro Athayde Marcondes de Andr\'{e}$^{45}$,
Didier Auguste$^{43}$,
Andrej Babic$^{70}$,
Wander Baldini$^{56}$,
Andrea Barresi$^{58}$,
Eric Baussan$^{45}$,
Marco Bellato$^{60}$,
Antonio Bergnoli$^{60}$,
Enrico Bernieri$^{64}$,
Thilo Birkenfeld$^{48}$,
Sylvie Blin$^{43}$,
David Blum$^{54}$,
Simon Blyth$^{40}$,
Anastasia Bolshakova$^{67}$,
Mathieu Bongrand$^{47}$,
Cl\'{e}ment Bordereau$^{44,39}$,
Dominique Breton$^{43}$,
Augusto Brigatti$^{57}$,
Riccardo Brugnera$^{61}$,
Riccardo Bruno$^{55}$,
Antonio Budano$^{64}$,
Mario Buscemi$^{55}$,
Jose Busto$^{46}$,
Ilya Butorov$^{67}$,
Anatael Cabrera$^{43}$,
Hao Cai$^{34}$,
Xiao Cai$^{10}$,
Yanke Cai$^{10}$,
Zhiyan Cai$^{10}$,
Antonio Cammi$^{59}$,
Agustin Campeny$^{5}$,
Chuanya Cao$^{10}$,
Guofu Cao$^{10}$,
Jun Cao$^{10}$,
Rossella Caruso$^{55}$,
C\'{e}dric Cerna$^{44}$,
Jinfan Chang$^{10}$,
Yun Chang$^{39}$,
Pingping Chen$^{18}$,
Po-An Chen$^{40}$,
Shaomin Chen$^{13}$,
Xurong Chen$^{26}$,
Yi-Wen Chen$^{38}$,
Yixue Chen$^{11}$,
Yu Chen$^{20}$,
Zhang Chen$^{10}$,
Jie Cheng$^{10}$,
Yaping Cheng$^{7}$,
Alexey Chetverikov$^{67}$,
Davide Chiesa$^{58}$,
Pietro Chimenti$^{3}$,
Artem Chukanov$^{67}$,
G\'{e}rard Claverie$^{44}$,
Catia Clementi$^{62}$,
Barbara Clerbaux$^{2}$,
Selma Conforti Di Lorenzo$^{43}$,
Daniele Corti$^{60}$,
Salvatore Costa$^{55}$,
Flavio Dal Corso$^{60}$,
Olivia Dalager$^{74}$,
Christophe De La Taille$^{43}$,
Jiawei Deng$^{34}$,
Zhi Deng$^{13}$,
Ziyan Deng$^{10}$,
Wilfried Depnering$^{52}$,
Marco Diaz$^{5}$,
Xuefeng Ding$^{57}$,
Yayun Ding$^{10}$,
Bayu Dirgantara$^{73}$,
Sergey Dmitrievsky$^{67}$,
Tadeas Dohnal$^{41}$,
Dmitry Dolzhikov$^{67}$,
Georgy Donchenko$^{69}$,
Jianmeng Dong$^{13}$,
Evgeny Doroshkevich$^{68}$,
Marcos Dracos$^{45}$,
Fr\'{e}d\'{e}ric Druillole$^{44}$,
Shuxian Du$^{37}$,
Stefano Dusini$^{60}$,
Martin Dvorak$^{41}$,
Timo Enqvist$^{42}$,
Heike Enzmann$^{52}$,
Andrea Fabbri$^{64}$,
Lukas Fajt$^{70}$,
Donghua Fan$^{24}$,
Lei Fan$^{10}$,
Can Fang$^{28}$,
Jian Fang$^{10}$,
Wenxing Fang$^{10}$,
Marco Fargetta$^{55}$,
Dmitry Fedoseev$^{67}$,
Vladko Fekete$^{70}$,
Li-Cheng Feng$^{38}$,
Qichun Feng$^{21}$,
Richard Ford$^{57}$,
Andrey Formozov$^{57}$,
Am\'{e}lie Fournier$^{44}$,
Haonan Gan$^{32}$,
Feng Gao$^{48}$,
Alberto Garfagnini$^{61}$,
Christoph Genster$^{50}$,
Marco Giammarchi$^{57}$,
Agnese Giaz$^{61}$,
Nunzio Giudice$^{55}$,
Maxim Gonchar$^{67}$,
Guanghua Gong$^{13}$,
Hui Gong$^{13}$,
Oleg Gorchakov$^{67}$,
Yuri Gornushkin$^{67}$,
Alexandre G\"{o}ttel$^{50,48}$,
Marco Grassi$^{61}$,
Christian Grewing$^{51}$,
Vasily Gromov$^{67}$,
Minghao Gu$^{10}$,
Xiaofei Gu$^{37}$,
Yu Gu$^{19}$,
Mengyun Guan$^{10}$,
Nunzio Guardone$^{55}$,
Maria Gul$^{66}$,
Cong Guo$^{10}$,
Jingyuan Guo$^{20}$,
Wanlei Guo$^{10}$,
Xinheng Guo$^{8}$,
Yuhang Guo$^{35,50}$,
Paul Hackspacher$^{52}$,
Caren Hagner$^{49}$,
Ran Han$^{7}$,
Yang Han$^{43}$,
Muhammad Sohaib Hassan$^{66}$,
Miao He$^{10}$,
Wei He$^{10}$,
Tobias Heinz$^{54}$,
Patrick Hellmuth$^{44}$,
Yuekun Heng$^{10}$,
Rafael Herrera$^{5}$,
Daojin Hong$^{28}$,
YuenKeung Hor$^{20}$,
Shaojing Hou$^{10}$,
Yee Hsiung$^{40}$,
Bei-Zhen Hu$^{40}$,
Hang Hu$^{20}$,
Jianrun Hu$^{10}$,
Jun Hu$^{10}$,
Shouyang Hu$^{9}$,
Tao Hu$^{10}$,
Zhuojun Hu$^{20}$,
Chunhao Huang$^{20}$,
Guihong Huang$^{10}$,
Hanxiong Huang$^{9}$,
Qinhua Huang$^{45}$,
Wenhao Huang$^{25}$,
Xin Huang$^{10}$,
Xingtao Huang$^{25}$,
Yongbo Huang$^{28}$,
Jiaqi Hui$^{30}$,
Lei Huo$^{21}$,
Wenju Huo$^{22}$,
C\'{e}dric Huss$^{44}$,
Safeer Hussain$^{66}$,
Antonio Insolia$^{55}$,
Ara Ioannisian$^{1}$,
Roberto Isocrate$^{60}$,
Beatrice Jelmini$^{61}$,
Kuo-Lun Jen$^{38}$,
Ignacio Jeria$^{5}$,
Xiaolu Ji$^{10}$,
Xingzhao Ji$^{20}$,
Huihui Jia$^{33}$,
Junji Jia$^{34}$,
Siyu Jian$^{9}$,
Di Jiang$^{22}$,
Xiaoshan Jiang$^{10}$,
Ruyi Jin$^{10}$,
Xiaoping Jing$^{10}$,
C\'{e}cile Jollet$^{44}$,
Jari Joutsenvaara$^{42}$,
Sirichok Jungthawan$^{73}$,
Leonidas Kalousis$^{45}$,
Philipp Kampmann$^{50}$,
Li Kang$^{18}$,
Michael Karagounis$^{51}$,
Narine Kazarian$^{1}$,
Waseem Khan$^{35}$,
Khanchai Khosonthongkee$^{73}$,
Denis Korablev$^{67}$,
Konstantin Kouzakov$^{69}$,
Alexey Krasnoperov$^{67}$,
Zinovy Krumshteyn$^{67}$,
Andre Kruth$^{51}$,
Nikolay Kutovskiy$^{67}$,
Pasi Kuusiniemi$^{42}$,
Tobias Lachenmaier$^{54}$,
Cecilia Landini$^{57}$,
S\'{e}bastien Leblanc$^{44}$,
Victor Lebrin$^{47}$,
Frederic Lefevre$^{47}$,
Ruiting Lei$^{18}$,
Rupert Leitner$^{41}$,
Jason Leung$^{38}$,
Demin Li$^{37}$,
Fei Li$^{10}$,
Fule Li$^{13}$,
Haitao Li$^{20}$,
Huiling Li$^{10}$,
Jiaqi Li$^{20}$,
Mengzhao Li$^{10}$,
Min Li$^{11}$,
Nan Li$^{10}$,
Nan Li$^{16}$,
Qingjiang Li$^{16}$,
Ruhui Li$^{10}$,
Shanfeng Li$^{18}$,
Tao Li$^{20}$,
Weidong Li$^{10,14}$,
Weiguo Li$^{10}$,
Xiaomei Li$^{9}$,
Xiaonan Li$^{10}$,
Xinglong Li$^{9}$,
Yi Li$^{18}$,
Yufeng Li$^{10}$,
Zhaohan Li$^{10}$,
Zhibing Li$^{20}$,
Ziyuan Li$^{20}$,
Hao Liang$^{9}$,
Hao Liang$^{22}$,
Jingjing Liang$^{28}$,
Daniel Liebau$^{51}$,
Ayut Limphirat$^{73}$,
Sukit Limpijumnong$^{73}$,
Guey-Lin Lin$^{38}$,
Shengxin Lin$^{18}$,
Tao Lin$^{10}$,
Jiajie Ling$^{20}$,
Ivano Lippi$^{60}$,
Fang Liu$^{11}$,
Haidong Liu$^{37}$,
Hongbang Liu$^{28}$,
Hongjuan Liu$^{23}$,
Hongtao Liu$^{20}$,
Hui Liu$^{19}$,
Jianglai Liu$^{30,31}$,
Jinchang Liu$^{10}$,
Min Liu$^{23}$,
Qian Liu$^{14}$,
Qin Liu$^{22}$,
Runxuan Liu$^{50,48}$,
Shuangyu Liu$^{10}$,
Shubin Liu$^{22}$,
Shulin Liu$^{10}$,
Xiaowei Liu$^{20}$,
Xiwen Liu$^{28}$,
Yan Liu$^{10}$,
Yunzhe Liu$^{10}$,
Alexey Lokhov$^{69,68}$,
Paolo Lombardi$^{57}$,
Claudio Lombardo$^{55}$,
Kai Loo$^{52}$,
Chuan Lu$^{32}$,
Haoqi Lu$^{10}$,
Jingbin Lu$^{15}$,
Junguang Lu$^{10}$,
Shuxiang Lu$^{37}$,
Xiaoxu Lu$^{10}$,
Bayarto Lubsandorzhiev$^{68}$,
Sultim Lubsandorzhiev$^{68}$,
Livia Ludhova$^{50,48}$,
Fengjiao Luo$^{10}$,
Guang Luo$^{20}$,
Pengwei Luo$^{20}$,
Shu Luo$^{36}$,
Wuming Luo$^{10}$,
Vladimir Lyashuk$^{68}$,
Bangzheng Ma$^{25}$,
Qiumei Ma$^{10}$,
Si Ma$^{10}$,
Xiaoyan Ma$^{10}$,
Xubo Ma$^{11}$,
Jihane Maalmi$^{43}$,
Yury Malyshkin$^{67}$,
Fabio Mantovani$^{56}$,
Francesco Manzali$^{61}$,
Xin Mao$^{7}$,
Yajun Mao$^{12}$,
Stefano M. Mari$^{64}$,
Filippo Marini$^{61}$,
Sadia Marium$^{66}$,
Cristina Martellini$^{64}$,
Gisele Martin-Chassard$^{43}$,
Agnese Martini$^{63}$,
Davit Mayilyan$^{1}$,
Ints Mednieks$^{65}$,
Yue Meng$^{30}$,
Anselmo Meregaglia$^{44}$,
Emanuela Meroni$^{57}$,
David Meyh\"{o}fer$^{49}$,
Mauro Mezzetto$^{60}$,
Jonathan Miller$^{6}$,
Lino Miramonti$^{57}$,
Salvatore Monforte$^{55}$,
Paolo Montini$^{64}$,
Michele Montuschi$^{56}$,
Axel M\"{u}ller$^{54}$,
Pavithra Muralidharan$^{51}$,
Massimiliano Nastasi$^{58}$,
Dmitry V. Naumov$^{67}$,
Elena Naumova$^{67}$,
Diana Navas-Nicolas$^{43}$,
Igor Nemchenok$^{67}$,
Minh Thuan Nguyen Thi$^{38}$,
Feipeng Ning$^{10}$,
Zhe Ning$^{10}$,
Hiroshi Nunokawa$^{4}$,
Lothar Oberauer$^{53}$,
Juan Pedro Ochoa-Ricoux$^{74,5}$,
Alexander Olshevskiy$^{67}$,
Domizia Orestano$^{64}$,
Fausto Ortica$^{62}$,
Rainer Othegraven$^{52}$,
Hsiao-Ru Pan$^{40}$,
Alessandro Paoloni$^{63}$,
Nina Parkalian$^{51}$,
Sergio Parmeggiano$^{57}$,
Yatian Pei$^{10}$,
Nicomede Pelliccia$^{62}$,
Anguo Peng$^{23}$,
Haiping Peng$^{22}$,
Fr\'{e}d\'{e}ric Perrot$^{44}$,
Pierre-Alexandre Petitjean$^{2}$,
Fabrizio Petrucci$^{64}$,
Oliver Pilarczyk$^{52}$,
Luis Felipe Pi\~{n}eres Rico$^{45}$,
Artyom Popov$^{69}$,
Pascal Poussot$^{45}$,
Wathan Pratumwan$^{73}$,
Ezio Previtali$^{58}$,
Fazhi Qi$^{10}$,
Ming Qi$^{27}$,
Sen Qian$^{10}$,
Xiaohui Qian$^{10}$,
Zhen Qian$^{20}$,
Hao Qiao$^{12}$,
Zhonghua Qin$^{10}$,
Shoukang Qiu$^{23}$,
Muhammad Usman Rajput$^{66}$,
Gioacchino Ranucci$^{57}$,
Neill Raper$^{20}$,
Alessandra Re$^{57}$,
Henning Rebber$^{49}$,
Abdel Rebii$^{44}$,
Bin Ren$^{18}$,
Jie Ren$^{9}$,
Taras Rezinko$^{67}$,
Barbara Ricci$^{56}$,
Markus Robens$^{51}$,
Mathieu Roche$^{44}$,
Narongkiat Rodphai$^{71}$,
Aldo Romani$^{62}$,
Bed\v{r}ich Roskovec$^{74}$,
Christian Roth$^{51}$,
Xiangdong Ruan$^{28}$,
Xichao Ruan$^{9}$,
Saroj Rujirawat$^{73}$,
Arseniy Rybnikov$^{67}$,
Andrey Sadovsky$^{67}$,
Paolo Saggese$^{57}$,
Giuseppe Salamanna$^{64}$,
Simone Sanfilippo$^{64}$,
Anut Sangka$^{72}$,
Nuanwan Sanguansak$^{73}$,
Utane Sawangwit$^{72}$,
Julia Sawatzki$^{53}$,
Fatma Sawy$^{61}$,
Michaela Schever$^{50,48}$,
Jacky Schuler$^{45}$,
C\'{e}dric Schwab$^{45}$,
Konstantin Schweizer$^{53}$,
Alexandr Selyunin$^{67}$,
Andrea Serafini$^{56}$,
Giulio Settanta$^{50}$,
Mariangela Settimo$^{47}$,
Zhuang Shao$^{35}$,
Vladislav Sharov$^{67}$,
Arina Shaydurova$^{67}$,
Jingyan Shi$^{10}$,
Yanan Shi$^{10}$,
Vitaly Shutov$^{67}$,
Andrey Sidorenkov$^{68}$,
Fedor \v{S}imkovic$^{70}$,
Chiara Sirignano$^{61}$,
Jaruchit Siripak$^{73}$,
Monica Sisti$^{58}$,
Maciej Slupecki$^{42}$,
Mikhail Smirnov$^{20}$,
Oleg Smirnov$^{67}$,
Thiago Sogo-Bezerra$^{47}$,
Sergey Sokolov$^{67}$,
Julanan Songwadhana$^{73}$,
Boonrucksar Soonthornthum$^{72}$,
Albert Sotnikov$^{67}$,
Ond\v{r}ej \v{S}r\'{a}mek$^{41}$,
Warintorn Sreethawong$^{73}$,
Achim Stahl$^{48}$,
Luca Stanco$^{60}$,
Konstantin Stankevich$^{69}$,
Du\v{s}an \v{S}tef\'{a}nik$^{70}$,
Hans Steiger$^{52,53}$,
Jochen Steinmann$^{48}$,
Tobias Sterr$^{54}$,
Matthias Raphael Stock$^{53}$,
Virginia Strati$^{56}$,
Alexander Studenikin$^{69}$,
Gongxing Sun$^{10}$,
Shifeng Sun$^{11}$,
Xilei Sun$^{10}$,
Yongjie Sun$^{22}$,
Yongzhao Sun$^{10}$,
Narumon Suwonjandee$^{71}$,
Michal Szelezniak$^{45}$,
Jian Tang$^{20}$,
Qiang Tang$^{20}$,
Quan Tang$^{23}$,
Xiao Tang$^{10}$,
Alexander Tietzsch$^{54}$,
Igor Tkachev$^{68}$,
Tomas Tmej$^{41}$,
Marco Danilo Claudio Torri$^{57}$,
Konstantin Treskov$^{67}$,
Andrea Triossi$^{45}$,
Giancarlo Troni$^{5}$,
Wladyslaw Trzaska$^{42}$,
Cristina Tuve$^{55}$,
Nikita Ushakov$^{68}$,
Johannes van den Boom$^{51}$,
Stefan van Waasen$^{51}$,
Guillaume Vanroyen$^{47}$,
Nikolaos Vassilopoulos$^{10}$,
Vadim Vedin$^{65}$,
Giuseppe Verde$^{55}$,
Maxim Vialkov$^{69}$,
Benoit Viaud$^{47}$,
Moritz Vollbrecht$^{50,48}$,
Cristina Volpe$^{43}$,
Vit Vorobel$^{41}$,
Dmitriy Voronin$^{68}$,
Lucia Votano$^{63}$,
Pablo Walker$^{5}$,
Caishen Wang$^{18}$,
Chung-Hsiang Wang$^{39}$,
En Wang$^{37}$,
Guoli Wang$^{21}$,
Jian Wang$^{22}$,
Jun Wang$^{20}$,
Kunyu Wang$^{10}$,
Lu Wang$^{10}$,
Meifen Wang$^{10}$,
Meng Wang$^{23}$,
Meng Wang$^{25}$,
Ruiguang Wang$^{10}$,
Siguang Wang$^{12}$,
Wei Wang$^{27}$,
Wei Wang$^{20}$,
Wenshuai Wang$^{10}$,
Xi Wang$^{16}$,
Xiangyue Wang$^{20}$,
Yangfu Wang$^{10}$,
Yaoguang Wang$^{34}$,
Yi Wang$^{13}$,
Yi Wang$^{24}$,
Yifang Wang$^{10}$,
Yuanqing Wang$^{13}$,
Yuman Wang$^{27}$,
Zhe Wang$^{13}$,
Zheng Wang$^{10}$,
Zhimin Wang$^{10}$,
Zongyi Wang$^{13}$,
Muhammad Waqas$^{66}$,
Apimook Watcharangkool$^{72}$,
Lianghong Wei$^{10}$,
Wei Wei$^{10}$,
Wenlu Wei$^{10}$,
Yadong Wei$^{18}$,
Liangjian Wen$^{10}$,
Christopher Wiebusch$^{48}$,
Steven Chan-Fai Wong$^{20}$,
Bjoern Wonsak$^{49}$,
Diru Wu$^{10}$,
Fangliang Wu$^{27}$,
Qun Wu$^{25}$,
Wenjie Wu$^{34}$,
Zhi Wu$^{10}$,
Michael Wurm$^{52}$,
Jacques Wurtz$^{45}$,
Christian Wysotzki$^{48}$,
Yufei Xi$^{32}$,
Dongmei Xia$^{17}$,
Yuguang Xie$^{10}$,
Zhangquan Xie$^{10}$,
Zhizhong Xing$^{10}$,
Benda Xu$^{13}$,
Cheng Xu$^{23}$,
Donglian Xu$^{31,30}$,
Fanrong Xu$^{19}$,
Hangkun Xu$^{10}$,
Jilei Xu$^{10}$,
Jing Xu$^{8}$,
Meihang Xu$^{10}$,
Yin Xu$^{33}$,
Yu Xu$^{50,48}$,
Baojun Yan$^{10}$,
Taylor Yan$^{73}$,
Wenqi Yan$^{10}$,
Xiongbo Yan$^{10}$,
Yupeng Yan$^{73}$,
Anbo Yang$^{10}$,
Changgen Yang$^{10}$,
Huan Yang$^{10}$,
Jie Yang$^{37}$,
Lei Yang$^{18}$,
Xiaoyu Yang$^{10}$,
Yifan Yang$^{10}$,
Yifan Yang$^{2}$,
Haifeng Yao$^{10}$,
Zafar Yasin$^{66}$,
Jiaxuan Ye$^{10}$,
Mei Ye$^{10}$,
Ziping Ye$^{31}$,
Ugur Yegin$^{51}$,
Fr\'{e}d\'{e}ric Yermia$^{47}$,
Peihuai Yi$^{10}$,
Na Yin$^{25}$,
Xiangwei Yin$^{10}$,
Zhengyun You$^{20}$,
Boxiang Yu$^{10}$,
Chiye Yu$^{18}$,
Chunxu Yu$^{33}$,
Hongzhao Yu$^{20}$,
Miao Yu$^{34}$,
Xianghui Yu$^{33}$,
Zeyuan Yu$^{10}$,
zezhong Yu$^{10}$,
Chengzhuo Yuan$^{10}$,
Ying Yuan$^{12}$,
Zhenxiong Yuan$^{13}$,
Ziyi Yuan$^{34}$,
Baobiao Yue$^{20}$,
Noman Zafar$^{66}$,
Andre Zambanini$^{51}$,
Vitalii Zavadskyi$^{67}$,
Shan Zeng$^{10}$,
Tingxuan Zeng$^{10}$,
Yuda Zeng$^{20}$,
Liang Zhan$^{10}$,
Aiqiang Zhang$^{13}$,
Feiyang Zhang$^{30}$,
Guoqing Zhang$^{10}$,
Haiqiong Zhang$^{10}$,
Honghao Zhang$^{20}$,
Jiawen Zhang$^{10}$,
Jie Zhang$^{10}$,
Jingbo Zhang$^{21}$,
Jinnan Zhang$^{10}$,
Peng Zhang$^{10}$,
Qingmin Zhang$^{35}$,
Shiqi Zhang$^{20}$,
Shu Zhang$^{20}$,
Tao Zhang$^{30}$,
Xiaomei Zhang$^{10}$,
Xuantong Zhang$^{10}$,
Xueyao Zhang$^{25}$,
Yan Zhang$^{10}$,
Yinhong Zhang$^{10}$,
Yiyu Zhang$^{10}$,
Yongpeng Zhang$^{10}$,
Yuanyuan Zhang$^{30}$,
Yumei Zhang$^{20}$,
Zhenyu Zhang$^{34}$,
Zhijian Zhang$^{18}$,
Fengyi Zhao$^{26}$,
Jie Zhao$^{10}$,
Rong Zhao$^{20}$,
Shujun Zhao$^{37}$,
Tianchi Zhao$^{10}$,
Dongqin Zheng$^{19}$,
Hua Zheng$^{18}$,
Minshan Zheng$^{9}$,
Yangheng Zheng$^{14}$,
Weirong Zhong$^{19}$,
Jing Zhou$^{9}$,
Li Zhou$^{10}$,
Nan Zhou$^{22}$,
Shun Zhou$^{10}$,
tong Zhou$^{10}$,
Xiang Zhou$^{34}$,
Jiang Zhu$^{20}$,
Kangpu Zhu$^{35}$,
Kejun Zhu$^{10}$,
ZhiHang Zhu$^{10}$,
Bo Zhuang$^{10}$,
Honglin Zhuang$^{10}$,
Liang Zong$^{13}$,
Jiaheng Zou$^{10}$
\\
$^{1}$Yerevan Physics Institute, Yerevan, Armenia.
$^{2}$Universit\'{e} Libre de Bruxelles, Brussels, Belgium.
$^{3}$Universidade Estadual de Londrina, Londrina, Brazil.
$^{4}$Pontificia Universidade Catolica do Rio de Janeiro, Rio, Brazil.
$^{5}$Pontificia Universidad Cat\'{o}lica de Chile, Santiago, Chile.
$^{6}$Universidad Tecnica Federico Santa Maria, Valparaiso, Chile.
$^{7}$Beijing Institute of Spacecraft Environment Engineering, Beijing, China.
$^{8}$Beijing Normal University, Beijing, China.
$^{9}$China Institute of Atomic Energy, Beijing, China.
$^{10}$Institute of High Energy Physics, Beijing, China.
$^{11}$North China Electric Power University, Beijing, China.
$^{12}$School of Physics, Peking University, Beijing, China.
$^{13}$Tsinghua University, Beijing, China.
$^{14}$University of Chinese Academy of Sciences, Beijing, China.
$^{15}$Jilin University, Changchun, China.
$^{16}$College of Electronic Science and Engineering, National University of Defense Technology, Changsha, China.
$^{17}$Chongqing University, Chongqing, China.
$^{18}$Dongguan University of Technology, Dongguan, China.
$^{19}$Jinan University, Guangzhou, China.
$^{20}$Sun Yat-Sen University, Guangzhou, China.
$^{21}$Harbin Institute of Technology, Harbin, China.
$^{22}$University of Science and Technology of China, Hefei, China.
$^{23}$The Radiochemistry and Nuclear Chemistry Group in University of South China, Hengyang, China.
$^{24}$Wuyi University, Jiangmen, China.
$^{25}$Shandong University, Jinan, China, and Key Laboratory of Particle Physics and Particle Irradiation of Ministry of Education, Shandong University, Qingdao, China.
$^{26}$Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, China.
$^{27}$Nanjing University, Nanjing, China.
$^{28}$Guangxi University, Nanning, China.
$^{29}$East China University of Science and Technology, Shanghai, China.
$^{30}$School of Physics and Astronomy, Shanghai Jiao Tong University, Shanghai, China.
$^{31}$Tsung-Dao Lee Institute, Shanghai Jiao Tong University, Shanghai, China.
$^{32}$Institute of Hydrogeology and Environmental Geology, Chinese Academy of Geological Sciences, Shijiazhuang, China.
$^{33}$Nankai University, Tianjin, China.
$^{34}$Wuhan University, Wuhan, China.
$^{35}$Xi'an Jiaotong University, Xi'an, China.
$^{36}$Xiamen University, Xiamen, China.
$^{37}$School of Physics and Microelectronics, Zhengzhou University, Zhengzhou, China.
$^{38}$Institute of Physics National Chiao-Tung University, Hsinchu.
$^{39}$National United University, Miao-Li.
$^{40}$Department of Physics, National Taiwan University, Taipei.
$^{41}$Charles University, Faculty of Mathematics and Physics, Prague, Czech Republic.
$^{42}$University of Jyvaskyla, Department of Physics, Jyvaskyla, Finland.
$^{43}$IJCLab, Universit\'{e} Paris-Saclay, CNRS/IN2P3, 91405 Orsay, France.
$^{44}$Univ. Bordeaux, CNRS, CENBG, UMR 5797, F-33170 Gradignan, France.
$^{45}$IPHC, Universit\'{e} de Strasbourg, CNRS/IN2P3, F-67037 Strasbourg, France.
$^{46}$Centre de Physique des Particules de Marseille, Marseille, France.
$^{47}$SUBATECH, Universit\'{e} de Nantes,  IMT Atlantique, CNRS-IN2P3, Nantes, France.
$^{48}$III. Physikalisches Institut B, RWTH Aachen University, Aachen, Germany.
$^{49}$Institute of Experimental Physics, University of Hamburg, Hamburg, Germany.
$^{50}$Forschungszentrum J\"{u}lich GmbH, Nuclear Physics Institute IKP-2, J\"{u}lich, Germany.
$^{51}$Forschungszentrum J\"{u}lich GmbH, Central Institute of Engineering, Electronics and Analytics - Electronic Systems (ZEA-2), J\"{u}lich, Germany.
$^{52}$Institute of Physics, Johannes-Gutenberg Universit\"{a}t Mainz, Mainz, Germany.
$^{53}$Technische Universit\"{a}t M\"{u}nchen, M\"{u}nchen, Germany.
$^{54}$Eberhard Karls Universit\"{a}t T\"{u}bingen, Physikalisches Institut, T\"{u}bingen, Germany.
$^{55}$INFN Catania and Dipartimento di Fisica e Astronomia dell Universit\`{a} di Catania, Catania, Italy.
$^{56}$Department of Physics and Earth Science, University of Ferrara and INFN Sezione di Ferrara, Ferrara, Italy.
$^{57}$INFN Sezione di Milano and Dipartimento di Fisica dell Universit\`{a} di Milano, Milano, Italy.
$^{58}$INFN Milano Bicocca and University of Milano Bicocca, Milano, Italy.
$^{59}$INFN Milano Bicocca and Politecnico of Milano, Milano, Italy.
$^{60}$INFN Sezione di Padova, Padova, Italy.
$^{61}$Dipartimento di Fisica e Astronomia dell'Universit\`{a} di Padova and INFN Sezione di Padova, Padova, Italy.
$^{62}$INFN Sezione di Perugia and Dipartimento di Chimica, Biologia e Biotecnologie dell'Universit\`{a} di Perugia, Perugia, Italy.
$^{63}$Laboratori Nazionali di Frascati dell'INFN, Roma, Italy.
$^{64}$University of Roma Tre and INFN Sezione Roma Tre, Roma, Italy.
$^{65}$Institute of Electronics and Computer Science, Riga, Latvia.
$^{66}$Pakistan Institute of Nuclear Science and Technology, Islamabad, Pakistan.
$^{67}$Joint Institute for Nuclear Research, Dubna, Russia.
$^{68}$Institute for Nuclear Research of the Russian Academy of Sciences, Moscow, Russia.
$^{69}$Lomonosov Moscow State University, Moscow, Russia.
$^{70}$Comenius University Bratislava, Faculty of Mathematics, Physics and Informatics, Bratislava, Slovakia.
$^{71}$Department of Physics, Faculty of Science, Chulalongkorn University, Bangkok, Thailand.
$^{72}$National Astronomical Research Institute of Thailand, Chiang Mai, Thailand.
$^{73}$Suranaree University of Technology, Nakhon Ratchasima, Thailand.
$^{74}$Department of Physics and Astronomy, University of California, Irvine, California, USA.

